Out-distribution aware Self-training in an Open World Setting

Deep Learning heavily depends on large labeled datasets which limits further improvements. While unlabeled data is available in large amounts, in particular in image recognition, it does not fulfill the closed world assumption of semi-supervised learning that all unlabeled data are task-related. The goal of this paper is to leverage unlabeled data in an open world setting to further improve prediction performance. For this purpose, we introduce out-distribution aware self-training, which includes a careful sample selection strategy based on the confidence of the classifier. While normal self-training deteriorates prediction performance, our iterative scheme improves using up to 15 times the amount of originally labeled data. Moreover, our classifiers are by design out-distribution aware and can thus distinguish task-related inputs from unrelated ones.

==> figures/cifar_temperatures.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{cifar10_ssl_conf_targets_0}
\caption{CIFAR10}
\label{subfig:cifar10_temperature}
\end{subfigure}
\begin{subfigure}{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{cifar100_ssl_conf_targets_0}
\caption{CIFAR100}
\label{subfig:cifar100_temperature}
\end{subfigure}
\caption{Max confidence targets after rescaling}
\label{fig:cifar_test_error_iterations}
\end{figure}

==> figures/svhn_80m_samples.tex <==
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{svhn_80M_samples_run_2.pdf}
\caption{\ours SVHN samples selected from 80M. }
\label{fig:svhn_80m_samples}
\end{figure}

==> tables/ablation_cifar_hard_labels.tex <==
\begin{table}[]
    \newcolumntype{M}{>{\centering\arraybackslash}m{0.55cm}}
    \small
    \centering
    \begin{tabular}{|c|MMM|MMM|}
     \hhline{~|---|---|}
     \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\ours} &  \multicolumn{3}{c|}{Iterative OE}\\
     \hline
     \textbf{CIFAR10} & 1st & 2nd & 3rd & 1st & 2nd & 3rd\\
     \hline
     Test error & 2.15 & 2.01 & \textbf{1.88} & 2.52 & 2.83 & 2.73\\
     \hline
     CIFAR10.1 & 5.40 & \textbf{4.55} & 4.70 & 6.40 & 6.65 & 6.60\\
     \hline
     CIFAR10-C & 14.19 & 15.02 & 15.46 & 15.39 & 14.49 & \textbf{13.96}\\
     \hhline{=======}
     \textbf{CIFAR100} & 1st & 2nd & 3rd & 1st & 2nd & 3rd\\
     \hline
     Test error & 15.91 & 15.38 & \textbf{14.86} & 18.27 & 17.64 & 17.77\\%82.23\\
     \hline
     CIFAR100-C & 36.92 & 35.64 & \textbf{34.82} & 38.85 & 37.75 & 36.80\\
     \hline
    \end{tabular}
    \caption{Ablation study: Comparison of \ours to iterative self-training that enforces uniform confidence on $\U \setminus \I$ instead of using soft-labels.}
    \label{tab:ablation_cifar_hard_od}
\end{table}

==> tables/ablation_cifar_label_smoothing.tex <==
\begin{table}[]
    \newcolumntype{M}{>{\centering\arraybackslash}m{0.55cm}}
    \small
    \centering
    \begin{tabular}{|c|MMM|MMM|}
     \hhline{~|---|---|}
     \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\ours} &  \multicolumn{3}{c|}{No label smoothing}\\
     \hline
     \textbf{CIFAR10} & 1st & 2nd & 3rd & 1st & 2nd & 3rd\\
     \hline
     Test error & 2.15 & 2.01 & \textbf{1.88} & \\
     \hline
     CIFAR10.1 & 5.40 & \textbf{4.55} & 4.70 & \\
     \hline
     CIFAR10-C & 14.19 & 15.02 & 15.46 & \\
     \hhline{=======}
     \textbf{CIFAR100} & 1st & 2nd & 3rd & 1st & 2nd & 3rd\\
     \hline
     Test error & 15.91 & 15.38 & \textbf{14.86} &\\
     \hline
     CIFAR100-C & 36.92 & 35.64 & \textbf{34.82} &\\
     \hline
    \end{tabular}
    \caption{Comparison to \ours without label smoothing on $\U \setminus \I$. }
    \label{tab:ablation_cifar_label_smoothing}
\end{table}

==> tables/cifar10_resnet50_auc.tex <==
\begin{table}[]
    \centering
    % \begin{tabular}{|c||c|c|c|c|}
    %     \hline 
    %     \textbf{AUROC} & Base & 1st & 2nd & 3rd \\
    %     \hhline{|=#=|=|=|=|}
    %     \ours & 98.95 & 99.20 & 99.16 & 98.98\\
    %     \hline
    %     \base & 92.74 & 89.39 & 83.73 & 75.93\\ 
    %     \hline
    %     \baseod & 92.74 & 90.35 & 84.14 & 85.71\\
    %     \hline
    % \end{tabular}
    % \caption{CIFAR10}
    % \label{tab:cifar10_resnet_auc}
    \begin{tabular}{|c||c|c|c|c|}
        \hline 
        \textbf{AUROC} & Base & 1st & 2nd & 3rd \\
        \hhline{|=#=|=|=|=|}
        \ours & 91.76 & 93.42 & 93.28 & 92.49\\
        \hline
        \base & 82.91 & 81.20 & 76.68 & 74.83\\ 
        \hline
        \baseod & 82.91 & 81.36 & 77.57 & 73.74\\
        \hline
    \end{tabular}
    \caption{CIFAR100}
    \label{tab:cifar100_resnet_auc}
\end{table}



==> tables/cifar_resnet_accuracy.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c||c|c|c|c|}
        \hline 
        \textbf{Error} & Base & 1st & 2nd & 3rd \\
        \hhline{|=#=|=|=|=|}
        \ours & 3.19 & 2.15 & 2.01 & 1.88\\
        \hline
        \base & 3.89 & 3.14 & 3.2 & 3.54\\ 
        \hline
        \baseod & 3.89 & 3.18 & 3.04 & 3.07\\
        \hline
    \end{tabular}
    \caption{CIFAR10}
    \label{tab:cifar10_resnet_error}
    \begin{tabular}{|c||c|c|c|c|}
        \hline 
        \textbf{Error} & Base & 1st & 2nd & 3rd \\
        \hhline{|=#=|=|=|=|}
        \ours & 20.02 & 15.91 & 15.38 & 14.86\\
        \hline
        \base & 19.31 & 17.56 & 17.54 & 18.40\\ 
        \hline
        \baseod & 19.31 & 17.97 & 17.84 & 18.76\\
        \hline
    \end{tabular}
    \caption{CIFAR100}
    \label{tab:cifar100_resnet_error}
\end{table}



==> tables/svhn_teacher_analysis.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c||c|c|c|}
        \hline 
         & 1st & 2nd & 3rd \\
        \hhline{|=#=|=|=|}
        Total Samples & 250k & 446k & 534k\\
        \hline
        SVHN samples & 249k & 438k & 502k\\
        \hline
        80M samples & 1000 & 7366 & 31465\\ 
        \hline
        SVHN precision & 99.82 & 99.68 & 99.49\\
        \hline
    \end{tabular}
    \caption{SVHN teacher}
    \label{tab:svhn_teacher}
\end{table}


